Meta-Video: Efficient Standardized Evaluation for Video Understanding

Video understanding benchmarks are the primary yardstick for measuring progress in video-language modeling, and a growing body of work relies on them to claim improvements. The reported benchmark scores in these works, however, are almost always produced by frameworks (e.g., lmms eval) used as black boxes: certain evaluation choices like frame sampling, preprocessing, and input formatting are inherited from preset defaults and seldom inspected carefully. We show these unexamined choices are a major source of variance. Even for the same model checkpoint, evaluation configuration alone can shift accuracy by up to 19.5pp. Hence, it is unclear whether reported gains reflect genuine improvements in capability or differences in evaluation setup. Moreover, many benchmark samples offer little evidence of visual capability, since they can be answered without the video, and the full suites are expensive to evaluate. We address these issues in two parts. First, we curate existing suites for discriminability and efficiency, producing Meta-Video, a balanced 1,000-question benchmark over 791 videos spanning diverse tasks and durations, which largely preserves model rankings, at 5 times inference speedup for a full-frame count sweep experiment (4-128 frames). Second, we establish a standardized evaluation protocol by sweeping the configuration space to isolate choices that measurably affect results, distill them into best practices and reporting standards, and release reproducible reference scores across five models and seven benchmarks. We hope that the proposed evaluation framework and the Meta-Video benchmark will support video understanding research by providing a reproducible and efficient foundation to measure progress in a reliable way. Project page: https://soumyasj.github.io/meta-video/

==> tables/prompts.tex <==
\begin{table}[t]
\centering\small
\resizebox{\textwidth}{!}{%
\begin{tabular}{llr}
\toprule
ID & Prompt & Note \\
\midrule
P0 & \textbackslash emph\{each dataset's own\} & each source's own answer-format line (the lmms-eval default) \\
P1 & \textbackslash texttt\{\textbackslash nAnswer with the option's letter from the given choices directly.\} & leading newline \\
P2 & \textbackslash texttt\{Answer with the option's letter from the given choices directly.\textbackslash n\} & same sentence, trailing newline instead of leading \\
P3 & \textbackslash texttt\{\textbackslash nAnswer the question with the option letter\} & shorter, no full stop \\
P4 & \textbackslash texttt\{\textbackslash nRespond with a single letter and nothing else.\} & minimal, no mention of options \\
P5 & \textbackslash texttt\{\textbackslash nWatch the video and choose the correct option.\} & an instruction about the task, not about the answer format \\
P6 & \textbackslash texttt\{\textbackslash nThink step by step about what happens in the video, then end your reply with Answer: \} & chain of thought, answer tagged at the end \\
P7 & \textbackslash texttt\{\textbackslash nGo through the frames in order: 1) describe what happens in each segment, 2) note anything inconsistent, 3) then answer.\} & chain of thought over the frames in order \\
P8 & \textbackslash texttt\{\textbackslash nAnswer with only the final answer: the option letter, or the number for numeric questions. No explanation.\} & direct answer, also valid for the numeric VSI-Bench questions \\
P9 & \textbackslash texttt\{\textbackslash nThink step by step about what happens in the video, then end your reply with "Answer: " followed by only the option letter, or the number for numeric questions.\} & chain of thought, also valid for the numeric VSI-Bench questions \\
\bottomrule
\end{tabular}
}
\caption{Prompt settings.}
\label{tab:mvb-prompts}
\end{table}

